CT4Rec: Simple yet Effective Consistency Training for Sequential Recommendation

Sequential recommendation methods are increasingly important in cutting-edge recommender systems. Through leveraging historical records, the systems can capture user interests and perform recommendations accordingly. State-of-the-art sequential recommendation models proposed very recently combine contrastive learning techniques for obtaining high-quality user representations. Though effective and performing well, the models based on contrastive learning require careful selection of data augmentation methods and pretext tasks, efficient negative sampling strategies, and massive hyper-parameters validation. In this paper, we propose an ultra-simple alternative for obtaining better user representations and improving sequential recommendation performance. Specifically, we present a simple yet effective \textbf{C}onsistency \textbf{T}raining method for sequential \textbf{Rec}ommendation (CT4Rec) in which only two extra training objectives are utilized without any structural modifications and data augmentation. Experiments on three benchmark datasets and one large newly crawled industrial corpus demonstrate that our proposed method outperforms SOTA models by a large margin and with much less training time than these based on contrastive learning. Online evaluation on real-world content recommendation system also achieves 2.717\% improvement on the click-through rate and 3.679\% increase on the average click number per capita. Further exploration reveals that such a simple method has great potential for CTR prediction. Our code is available at \url{https://github.com/ct4rec/CT4Rec.git}.

==> Table/DataConsis.tex <==
\begin{table}[]
\caption{Experimental results of more consistency training.}\label{tab:data_consistency}
\begin{tabular}{ccccc}
  \toprule
Metrics  & SASRec* & CT4Rec & CT4Rec$^+$& Improv.$^+$\\
  \hline
HR@5  & 0.2194  & 0.2556 & \textbf{0.2582}          & 1.02\%               \\
HR@10  & 0.2748  & 0.3200 & \textbf{0.3253}          & 1.66\%               \\
HR@20   & 0.3392  & 0.3891 & \textbf{0.3975}          & 2.16\%               \\
NDCG@5  & 0.1661  & 0.1924 & \textbf{0.1927}          & 0.16\%               \\
NDCG@10  & 0.1840  & 0.2132 & \textbf{0.2143}          & 0.52\%               \\
NDCG@20  & 0.2003  & 0.2307 & \textbf{0.2325}          & 0.78\%    \\
         \bottomrule
\end{tabular}
\end{table}

==> Table/LayerDrop.tex <==
\begin{table}[]
\caption{CT4Rec with LayerDrop. The baseline model SASRec* also use LayerDrop instead of Dropout.}
\small
\begin{tabular}{lllll}
\hline
Dataset                 & Metric  & SASRec* & CT4Rec$^L$ & Improve* \\ \hline
\multirow{6}{*}{Beauty} & HR@5    & 0.1576 & 0.1707                 & 8.31\%  \\
                        & HR@10   & 0.2021 & 0.2171                 & 7.42\%  \\
                        & HR@20   & 0.2598 & 0.2765                 & 6.43\%  \\
                        & NDCG@5  & 0.1182 & 0.1295                 & 9.56\%  \\
                        & NDCG@10 & 0.1325 & 0.1445                 & 9.06\%  \\
                        & NDCG@20 & 0.1470 & 0.1595                 & 8.50\%  \\ \hline
\multirow{6}{*}{Sport}  & HR@5    & 0.1410 & 0.1510                 & 7.09\%  \\
                        & HR@10   & 0.1974 & 0.2085                 & 5.62\%  \\
                        & HR@20   & 0.2720 & 0.2825                 & 3.86\%  \\
                        & NDCG@5  & 0.0987 & 0.1074                 & 8.81\%  \\
                        & NDCG@10 & 0.1169 & 0.1258                 & 7.61\%  \\
                        & NDCG@20 & 0.1357 & 0.1445                 & 6.48\%  \\ \hline
\multirow{6}{*}{Yelp}   & HR@5    & 0.2342 & 0.2485                 & 6.11\%  \\
                        & HR@10   & 0.3464 & 0.3641                 & 5.11\%  \\
                        & HR@20   & 0.4921 & 0.5153                 & 4.71\%  \\
                        & NDCG@5  & 0.1606 & 0.1715                 & 6.79\%  \\
                        & NDCG@10 & 0.1967 & 0.2087                 & 6.10\%  \\
                        & NDCG@20 & 0.2334 & 0.2468                 & 5.74\%  \\ \hline
\multirow{6}{*}{Wechat} & HR@5    & 0.2304 & 0.2450                 & 6.34\%  \\
                        & HR@10   & 0.3437 & 0.3581                 & 4.19\%  \\
                        & HR@20   & 0.4823 & 0.5077                 & 5.26\%  \\
                        & NDCG@5  & 0.1561 & 0.1658                 & 6.21\%  \\
                        & NDCG@10 & 0.1887 & 0.2011                 & 6.57\%  \\
                        & NDCG@20 & 0.2194 & 0.2329                 & 6.15\%  \\ \hline
\end{tabular}
\label{tab:LayerDrop}
\end{table}


==> Table/reorder.tex <==
\begin{table}[th]
    \caption{Transformer reorder as model noise. \textit{Improv.*} and \textit{Improv.$^R$} refer to the relative improvement of CT4Rec$^R$ over SASRec* and CT4Rec, respectively.}
    % \centering
    \begin{tabular}{lllllll}
     \toprule
    Dataset   & Metric & SASRec* & CT4Rec  & CT4Rec$^R$ & Improv.* & Improv.$^R$  \\
    \hline
    Beauty & HR@5    & 0.2198~ & 0.2556~ & 0.2556~          & 16.29\% & 0.00\%    \\
           & HR@10   & 0.2740~ & 0.3200~ & 0.3202~          & 16.86\% & 0.06\%    \\
           & HR@20   & 0.3360~ & 0.3891~ & 0.3921~          & 16.70\% & 0.77\%    \\
           & NDCG@5  & 0.1674~ & 0.1924~ & 0.1914~          & 14.34\% & -0.52\%   \\
           & NDCG@10 & 0.1849~ & 0.2132~ & 0.2124~          & 14.87\% & -0.38\%   \\
           & NDCG@20 & 0.2005~ & 0.2307~ & 0.2305~          & 14.96\% & -0.09\%   \\
           \hline
    Sport  & HR@5    & 0.1985~ & 0.2196~ & 0.2203~          & 10.98\% & 0.32\%    \\
           & HR@10   & 0.2682~ & 0.3010~ & 0.3012~          & 12.30\% & 0.07\%    \\
           & HR@20   & 0.3545~ & 0.3950~ & 0.3946~          & 11.31\% & -0.10\%   \\
           & NDCG@5  & 0.1414~ & 0.1556~ & 0.1557~          & 10.11\% & 0.06\%    \\
           & NDCG@10 & 0.1639~ & 0.1817~ & 0.1817~          & 10.86\% & 0.00\%    \\
           & NDCG@20 & 0.1857~ & 0.2055~ & 0.2053~          & 10.55\% & -0.10\%   \\
           \hline
    Yelp   & HR@5    & 0.3210~ & 0.3462~ & 0.3486~          & 8.60\%  & 0.69\%    \\
           & HR@10   & 0.4477~ & 0.4784~ & 0.4805~          & 7.33\%  & 0.44\%    \\
           & HR@20   & 0.6004~ & 0.6309~ & 0.6341~          & 5.61\%  & 0.51\%    \\
           & NDCG@5  & 0.2275~ & 0.2443~ & 0.2460~          & 8.13\%  & 0.70\%    \\
           & NDCG@10 & 0.2684~ & 0.2869~ & 0.2885~          & 7.49\%  & 0.56\%    \\
           & NDCG@20 & 0.3068~ & 0.3253~ & 0.3273~          & 6.68\%  & 0.61\%   \\
            \hline
    Wechat & HR@5    & 0.3062~ & 0.3406~ & 0.3431~          & 12.05\%  & 0.73\%    \\
           & HR@10   & 0.4371~ & 0.4861~ & 0.4887~          & 11.80\%  & 0.53\%    \\
           & HR@20   & 0.5473~ & 0.5979~ & 0.5992~          & 9.48\%  & 0.22\%    \\
           & NDCG@5  & 0.2125~ & 0.2361~ & 0.2380~          & 12.00\%  & 0.81\%    \\
           & NDCG@10 & 0.2748~ & 0.3057~ & 0.3074~          & 11.86\%  & 0.56\%    \\
           & NDCG@20 & 0.3024~ & 0.3314~ & 0.3329~          & 10.09\%  & 0.45\%   \\
            \bottomrule
    \end{tabular}
    \label{tab:reorder}
\end{table}

==> Table/reorder_without_dropout.tex <==
\begin{table}
 \caption{Transformer reorder as model noise removing all dropout operations from both SASRec* and CT4Rec$^R$}
\centering
\small
\begin{tabular}{lllll}
 \toprule
Dataset   & Metric & SASRec* & CT4Rec$^R$ & Improv. \\
\hline
Beauty & HR@5    & 0.1573  & 0.1615 & 2.67\%   \\
       & HR@10   & 0.2035  & 0.2058 & 1.13\%   \\
       & HR@20   & 0.2620   & 0.2617 & -0.11\%  \\
       & NDCG@5  & 0.1190   & 0.1223 & 2.77\%   \\
       & NDCG@10 & 0.1339  & 0.1365 & 1.94\%   \\
       & NDCG@20 & 0.1486  & 0.1506 & 1.35\%  \\
        \bottomrule
\end{tabular}
 \label{tab:reorder_wod}
\end{table}
